Classification Protocols with Minimal Disclosure

We consider multi-party protocols for classification that are motivated by applications such as e-discovery in court proceedings. We identify a protocol that guarantees that the requesting party receives all responsive documents and the sending party discloses the minimal amount of non-responsive documents necessary to prove that all responsive documents have been received. This protocol can be embedded in a machine learning framework that enables automated labeling of points and the resulting multi-party protocol is equivalent to the standard one-party classification problem (if the one-party classification problem satisfies a natural independence-of-irrelevant-alternatives property). Our formal guarantees focus on the case where there is a linear classifier that correctly partitions the documents.

==> cpp2-proof.tex <==
\newcommand{\XY}{\textrm{XY}}

Given labeled examples $A_+ \subseteq S_+$ and $A_- \subseteq S_-$, let us define 
$$\XY(A_+, A_-) \coloneqq A_+ \times \{+1\} \cup A_- \times \{-1\} \subset \R^n \times \{ \pm 1\} = \{(x,1),x\in A_+ \} \cup \{(-x,-1),x\in A_-\}. $$
Any hypothesis $h=\text{sign}(d\cdot x + c) \in \cH_{A_+, A_-}$ satisfies 
$$ \forall (x,y) \in \XY(A_+, A_-), ~~  y(d\cdot x +c)>0.$$
This motivates the definition of the following cone, where $\cone(T)$ consists of all non-negative linear combinations of the points in $T$:
\begin{align}
K_{A_+,A_-} &\coloneqq  \cone\big(\big\{(yx, y): (x,y) \in \XY(A_+, A_-\big\}\big) 
\end{align}
The following statement gives a simple characterization of $\Leak(A_+, A_-)$. 
%\[\Leak(A_+,A_-)=\{z\in S: (-z,-1)\not\in K_{A_+,A_-}\}\]
\begin{lemma}\label{lem:leakcone}
  For any $\Ap \subseteq \Sp$ and $\Am \subseteq \Sm$, we have  
  \begin{equation}
      \Leak(A_+,A_-)=\{z\in S: (-z,-1)\not\in K_{A_+,A_-}\}. \label{eq:leakcone}
  \end{equation}

\end{lemma}
\begin{proof}
Suppose $z \in \Leak(A_+, A_-)$. Then there exists $(d,c) \in \R^n \times \R$ s.t. 
\begin{align*}
 d \cdot (yx) + c y > 0 &~~    \forall (x,y) \in \XY(A_+, A_-),\\
\text{ but }~ d \cdot z + c >0 &~\implies~  d \cdot (-z) + c (-1) <0. 
\end{align*}
This shows that $(-z,-1) \notin K_{A_+, A_-}$. 

On the other hand, suppose $(-z,-1) \notin K_{A_+, A_-}$. By the hyperplane separator theorem there exists $(c,d) \in \R^n \times \R$ such that $-d \cdot z - c <0$,  but %$\forall u \in K_{A_+, A_-}, ~(c,d) \cdot u >0$. In particular 
$y(c \cdot x + d)  >0$ for all $(x,y) \in \XY(A_+, A_-)$. Hence $z \in \Leak(A_+, A_-)$.

\end{proof}

\begin{lemma}
  $K_{\Sp,\Am}=K_{\Sp,\Sm}$ for all $A_- \supseteq C^*(S_+)$. Moreover $K_{S_+, S_-}  K_{S_+, A_-}$ if and only if $A_-\supseteq C*(\Sp)$.
\end{lemma}
\begin{proof}
%We prove this claim inductively. 
% \begin{claim}
% For all $T \subseteq \Sm \setminus C^*(S_+)$, $K(\Sp, \Sm \setminus T) = K(\Sp, \Sm) $.
% \end{claim}
% We now prove the claim by induction on $|T|$. The base case is $|T|=0$, where it is clearly true. 

% Let $x^* \in T$. Let $S' = \Sm \setminus T$. By the induction hypothesis we have $K(\Sp, S' \cup \{x^*\} ) = K(\Sp, \Sm)$. We now show that $K(\Sp, S')= K(\Sp, \Sm)$. 

Suppose not for contradiction. There exists $z^* \in K(\Sp, \Sm) \setminus K(\Sp, \CP(\Sp))$, i.e., there exists $z^* \in \R^n \times \R$ such that 
\begin{align}
    z^* &\notin K(\Sp, \CP(\Sp)), \text{ while} \label{eq:onehand}\\
    z^* &= \sum_{x \in \Sm} \lambda_x (-x, -1) + \sum_{x \in \Sp} \lambda_x (x,1) ~\text{ for some } \lambda \in \mathbb{R}_{\ge 0}^{\Sm} \setminus \{0\} \nonumber \\
    &=\sum_{x \in \Sm \setminus \CP(\Sp)}\lambda_x (-x, -1) +z' \text{ for some } \lambda \in \mathbb{R}_{\ge 0}^{\Sm \setminus \CP(\Sp)} \setminus \{0\}, z' \in K(\Sp, \CP(\Sp)) \label{eq:otherhand}. 
\end{align}
Hence there is a hyperplane $(d,c) \in \R^n \times \R$ separating $z^*$ and $K(\Sp, \CP(\Sp))$ so that for some $z' \in K(\Sp, \CP(\Sp))$
\begin{align*}
\forall z \in K(\Sp, S'),    (d,c) \cdot z >0 & \text{ but } (d,c) \cdot \big( \lambda (-x^*, -1) + z' \big) \\
\text{Thus }    z = \lambda (-x^*, -1) +z' \text{ for some } \lambda >0, z' \in K(\Sp, S'), \text{ but } z \notin K(\Sp, S'). 
\end{align*}

\end{proof}

==> extrastuff.tex <==
\section*{Mar 7}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\begin{algorithm}
\caption{Single-party Information Retrieval (SPIR)}\label{alg:spir}
\begin{algorithmic}[1]
\Require unlabeled samples $U\subseteq \R^n$ and the hypothesis class $\cH$ such that $U$ is separable by $\cH$
\Ensure samples estimated to have the positive label $\hat{U}_+\subseteq U$.
\State Samples $S\subseteq U$ with $|S|\ll |U|$
\State (Hand-)Label $S$ and get $S_+$ and $S_-$.
\State Learn classifier $\hat{h}\in \cH$ using $S_+$ and $S_-$.
\State Apply $\hat{h}$ to $U$ and get $\hat{U}_+$
\end{algorithmic}
\end{algorithm}
Multi-party Information Retrieval (MPIR)
\begin{itemize}
	\item Alice
	\begin{enumerate}
		\item has $U$
		\item adversarial in order to hide files in $U$. Hiding a relevant file can be more beneficial than hiding an irrelevant one, but the assumption is not important for us.
	\end{enumerate}
	Bob
	\begin{enumerate}
		\item has query access to labels
		\item wants $\hat{U}_+$
		\item ``curious but honest''
	\end{enumerate}
	\item Naive approach 1: Alice does SPIR and sends $\hat{U}_+$ to Bob.
	\item Problem: Trust issue.\\Alice may hide from $\hat{U}_+$ and send a much smaller set than $\hat{U}_+$. There is no way for Bob to tell.
	\item Naive approach 2: Alice sends $U$ to Bob and let Bob do SPIR.
	\item Problem: Privacy concern.\\
	Most of $U$ are irrelevant and hence are Alice's rightful privacy, yet revealed to Bob in this approach.
	\item We need a mediator or trusted third party (TTP).
	\item Naive approach 3 (with TTP): TTP asks Alice for $U$ and Bob for a perfect classifier $h^*$ and does SPIR.
	\item Problem: Bob only has query access to the labels. Finding $h^*$ would be extremely costly if possible at all.
	\item Observation: Only step 2 of SPIR needs Bob.
	\item Naive approach 4 (with TTP): TTP asks Alice for $U$, samples $S\subseteq U$ with $|S|\ll |U|$ (step 1 of SPIR), sends $S$ to Bob. Bob (hand-)label $S$ and gets $S_+$ and $S_-$. Either Bob or TTP does step 3. Finally, TTP does step 4 and sends $\hat{U}_+$ to Bob.
	\item (Moderate) Problem: Bob still sees $S_-$.

		\begin{algorithm}
		\caption{Multi-party Information Retrieval (MPIR)}\label{alg:mpir}
		\begin{algorithmic}[1]
		% \Require $n \geq 0$
		% \Ensure $y = x^n$
		\State Alice sends $U$ to TTP
		\State TTP samples $S\subseteq U$ with $|S|\ll |U|$ (can be done by Bob by picking indices) and sends Alice $S$
		\State Alice picks $A_+\subseteq X$ and $A_-\subseteq X$ and sends them to TTP
		\State TTP ensures $A_+\subseteq S$ and $A_-\subseteq S$ and sends them to Bob
		\State Bob ensures $A_+$ all have label $+$ and $A_-$ all have label $-$ by hand-labeling.
		\If{Consistent}
		    \State TTP computes and sends to Bob all emails potentially relevant and hidden by Alice, namely
		    \[\Leak(A_+,A_-)=\{x\in S: \exists h\in\cH, h(x)>0 \text{ and consistent with }A_+ \text{ and } A_-\}.\]
		    \State Bob sets his set of observed files
		    $\obs=\Leak(A_+,A_-)\cup A_+ \cup A_-$
		    \djs{plus and minus notations...}
		    % \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
		\Else
			\State TTP sends $S$ to Bob
		    \State Bob sets his set of observed files $\obs=S\cup A_+ \cup A_-$
		\EndIf
		\State Bob hand-labels $\obs$, learns a classifier $\hat{h}\in \cH$ and sends $\hat{h}$ to TTP.
		\State TTP applies $\hat{h}$ to $U$ and sends $\hat{U}_+$ to Bob.
		% \State Bob verifies that $A_+$ and $A_-$ are consistent with $h^*$, i.e. $h^*(x_+)>0, \forall x_+\in A_+$ and $h^*(x_-)>0, \forall x_-\in A_-$, and sends the result to TTP.
		% \While{$N \neq 0$}
		% \EndWhile
		\end{algorithmic}
		\end{algorithm}

\end{itemize}
The goal of Alice \djs{Can Alice do something that affect the quality of $\hat{h}$?} is to minimize the number of files observed by Bob, i.e.
\[|\obs(A_+,A_-)|\tag{$*$}\]
where the variables are the two sets $A_+$ and $A_-$.
\begin{theorem}\label{thm:min:old}
	In the linear separable case, the minimizer of $(*)$ is $(S_+,A_-^*)$ where
    \[A_-^*=\{x\in S_-: \exists h\in\cH, h\mid_{S_-\backslash\{x\}}\leqslant0,h(x)=0,h\mid_{S_+}>0\}.\]
    In this case, $\obs(S_+,A_-^*)=S_+\cup A_-^*$.
\end{theorem}
In other words, in the linear separable case, Alice is incentivized by \Cref{alg:mpir} to give Bob exactly what he needs. \djs{elaborate}


% A binary classfication problem is a triplet $(S_+,S_-,\cH)$ .
For a binary classfication problem $(S_+,S_-,\cH)$ where $S_+\subseteq X$ and $S_-\subseteq X$ are the $+$ and $-$ datasets and $\cH\subseteq\{\pm\}^X$ is the hypothesis class, let $\cH_{S_+,S_-}=\{h\in\cH: h(x)=+,\forall x\in S_+,h(y)=-,\forall y\in S_-\}$ be the set of consistent hypothese.
The pair of datasets $(S_+,S_-)$ is said to be \emph{separable} by $\cH$ if there is a consistent hypothesis, i.e. $\cH_{S_+,S_-}\neq\varnothing$.
A learning algorithm $\cA_\cH$ for a hypothesis class $\cH$ takes the datasets as input and outputs a hypothesis in $\cH$.
\djs{$\cA: 2^X\times 2^X\times 2^{\{\pm\}^X}\to \{\pm\}^X$ might be too formal to be helpful.}

\begin{definition} \label{def:IIA:old}
	A learning algorithm $\cA_\cH$ is said to satisfy \emph{independence of irrelevant alternatives} (IIA) if the output hypothesis remains the same as long as the set of consistent hypotheses remains the same, i.e.
	\[\cH_{S_+,S_-}=\cH_{T_+,T_-}\implies \cA_\cH(S_+,S_-)=\cA_\cH(T_+,T_-).\]
\end{definition}
In particular, an IIA learning algorithm $\cA_\cH$ depends on the data only via $\cH_{S_+,S_-}$
\begin{theorem}\label{thm:IIA}
	In the linear separable case, \Cref{alg:spir,alg:mpir} with the same sampling procedure and IIA learning algorithm $\cA_\cH$ produces the same $\hat{U}_+$.
\end{theorem}
\begin{proof}[Proof of \Cref{thm:IIA}]
	By \Cref{thm:min}, Alice sends $S_+$ and $A_-^*$. It suffices to show that 
	$\cH_{S_+,S_-}=\cH_{S_+,A^*_-}$
\end{proof}
Because of the randomness in the sampling procedure and potentially in the learning algorithm $\cA_\cH$, $\hat{U}_+$ is a random set, so \Cref{thm:IIA} should be interpreted as the distributions of $\hat{U}_+$ are the same.


\begin{proof}[Proof of \Cref{thm:min}]
First observe that in the inconsistent case, $S\subseteq \obs=S\cup A_+ \cup A_-$, while in the consistent case, $\obs=\Leak(A_+,A_-)\cup A_+ \cup A_-\subseteq S$. So it is safe to assume that $A_+$ and $A_-$ are consistent, i.e. $A_+\subseteq S_+, A_-\subseteq S_-$. The rest is broken down into the following claims.

\begin{claim}$\phantom{a}$
\begin{enumerate}
	\item 
	For any $A_+\subseteq S_+, A_-\subseteq S_-$,
	$\obs(A_+,A_-)\supseteq \obs(S_+,A_-)$.
	\item For any $A_-\subseteq S_-$,
	$\obs(S_+,A_-)\supseteq S_+\cup A_-^*$
	\item 
	$\obs(S_+,A_-^*)= S_+\cup A_-^*$
\end{enumerate}
\end{claim}

Let $K_{A_+,A_-}=\cone\{(x,1),x\in A_+,(-y,-1),y\in A_-\}$.
\[\Leak(A_+,A_-)=\{z\in S: (-z,-1)\not\in K_{A_+,A_-}\}\]
% =S\cap(H^-_{A,B})^c
Let
\begin{align*}
	A_+^* &:= \{x^*\in S_+: \exists (c,d)\text{ s.t. } c^Tx^*+d=0\text{ and }c^Tx+d>0,\forall x\in S_+,x\neq x^*\text{ and }c^Ty+d<0,\forall y\in S_-\}\\
	A_-^* &:= \{y^*\in S_-: \exists (c,d)\text{ s.t. } c^Ty^*+d=0\text{ and }c^Ty+d<0,\forall y\in S_-,y\neq y^*\text{ and }c^Tx+d>0,\forall x\in S_+\}
\end{align*}


\begin{lemma}
	For any $A_+\subseteq S_+, A_-\subseteq S_-$,
	$\obs(A_+,A_-)=S_+\cup A_-$ if and only if $A_+\supseteq A_+^*$ and $A_-\supseteq A_-^*$
\end{lemma}
For a convex cone $C$, let $R(C)$ be the set of extreme rays of $C$. For a point $x$, let $\overline{x}=\{\lambda x: \lambda\geqslant0\}$ be the ray represented by $x$.
\begin{lemma}
	$R(K_{S_+,S_-}) = \{\overline{(x,1)}, \overline{(-y,-1)}: x\in A_+^*, y\in A_-^*\}$.
\end{lemma}
In particular, we have
\begin{corollary}\label{cor:coneK}
For $A_+\subseteq S_+, A_-\subseteq S_-$, 
	$K_{S_+,S_-}=K_{A_+,A_-}$ if and only if $A_+\supseteq A_+^*$ and $A_+\supseteq A_-^*$. In particular,
	% $K_{S_+,S_-}=K_{A^*_+,A^*_-}$ and 
	$\cH_{S_+,S_-}=\cH_{A^*_+,A^*_-}$
\end{corollary}

We know that the dual 
\begin{align*}
	K^*_{S_+,S_-}=\{(c,d)\in\R^{n+1}\mid c^Tx+d&\geqslant0,\forall x\in S_+\\
	c^Tx+d&\leqslant0,\forall y\in S_-\}
\end{align*}
consists of linear classifiers consistent with $S_+$ and $S_-$, i.e. $K^*_{S_+,S_-}=\cH_{S_+,S_-}$ 
Let
\begin{align*}
	H^+_{A,B}&=\{x:c^T x+d\geqslant 0, \forall (c,d)\in K^*_{A,B}\},\\
	H^-_{A,B}&=\{x:c^T x+d\leqslant 0, \forall (c,d)\in K^*_{A,B}\}
\end{align*}
\begin{align*}
	H^+_{A,B}&=\{x:(x,1)\in K_{A,B}\},\\
	H^-_{A,B}&=\{y:(-y,-1)\in K_{A,B}\}
\end{align*}
% Obviously, when $A\subseteq S_+, B\subseteq S_-$
	Observe that $K_{A,B}$ is increasing in both variables, hence $K^*_{A,B}$ is decreasing, hence $H^-_{A,B}$ is decreasing.

\begin{itemize}
	\item $\Leak(A_+,A_-)$ is decreasing in both variables
\end{itemize}
And because of realizability,
\begin{itemize}
	\item $\Leak(A_+,A_-)\supseteq S_+$
\end{itemize}
We have
\begin{align*}
	\Leak(A_+,A_-)\cup A_+ \cup A_-
	&=\Leak(A_+,A_-)\cup A_-\\
	&\supseteq\Leak(S_+,A_-)\cup A_-\\
	&=S_+\sqcup L(A_-)\sqcup A_-
\end{align*}
\end{proof}


\section*{Mar 5}
Let $K=\cone\{(x,1),x\in S_+,(-y,-1),y\in S_-\}$ and $\mathbb{H}=\{(x,t): t\geqslant0\}$. Let $K_+ = K\cap\mathbb{H}, K_-=K\cap(-\mathbb{H})$.
Then
\begin{lemma}
	$K_+=\cone\{(x,1): x\in H_+\}, K_-=\cone\{(x,-1): x\in H_-\}$.
\end{lemma}
For a convex cone $C$, let $R(C)$ be the set of extreme rays of $C$. For a point $x$, let $\overline{x}=\{\lambda x: \lambda\geqslant0\}$ be the ray represented by $x$.
\begin{lemma}
	$R(K) = \{\overline{(x,1)}, \overline{(-y,-1)}: x\in A_+^*, y\in A_-^*\}$.
\end{lemma}
\begin{proof}
	First notice that any ray in $K$ can be represented by a vector of the form $(z,1),(z,-1)$ or $(z,0)$.
	\begin{enumerate}
		\item 
		Suppose $(z,1)$ is extreme, this means there exists $(c,d)$ such that
		\begin{enumerate}
			\item $c^Tz+d=0$
			\item $c^Tu+dt\geqslant 0,\forall (u,t)\in K$.
			\item $c^Tu+dt=0, (u,t)\in K\implies t\geqslant0, u=tz$.
		\end{enumerate}
		The first two conditions mean $(z,1)$ supports a half-space that contains $K$. The third condition means $K$ intersects the hyperplane exactly at the ray.

		(b) is equivalent to that $c^Tx+d\geqslant 0,\forall x\in S_+,c^Ty+d\leqslant 0,\forall y\in S_-$.

		Consider $(u,t)$ in the intersection, i.e. $c^Tu+dt=0, (u,t)\in K$. We know
		$$\textstyle(u,t)=\sum_{x\in S_+} \lambda_x (x,1)+\sum_{y\in S_-} \gamma_y (-y,-1)\text{ where }\lambda_x\geqslant0,\gamma_y\geqslant0.$$
		% Hence $u=\sum_{x\in S_+} \lambda_x x-\sum_{y\in S_-} \gamma_y y$ and $t=\sum_{x\in S_+} \lambda_x-\sum_{y\in S_-} \gamma_y$ 
		Hence $u=\sum \lambda_x x-\sum \gamma_y y$ and $t=\sum \lambda_x-\sum \gamma_y$ where the obvious summation subscripts are dropped for brevity. $c^Tu+dt=0$ can be expanded as
		\begin{align*}\textstyle
			c^T\sum \lambda_x x-\sum \gamma_y y + d\cdot(\sum \lambda_x-\sum \gamma_y)=0
		\end{align*}
		\begin{align*}\textstyle
			\sum \lambda_x (c^Tx+d)=\sum \gamma_y (c^Ty + d) \tag{$*$}
		\end{align*}
		By (2), LHS of $(*)$ $\geqslant0$ and RHS of $(*)$ $\leqslant0$, which implies both are 0 and the coefficients can be positive only when the corresponding linear form evaluates to 0. More precisely, let $H=\{x:c^Tx+d=0\}$ be the hyperplane. We have
		\begin{align*}
			u&=\sum_{x\in S_+\cap H} \lambda_x x-\sum_{y\in S_-\cap H} \gamma_y y\\
			t&=\sum_{x\in S_+\cap H} \lambda_x-\sum_{y\in S_-\cap H} \gamma_y
		\end{align*}
		Moreover, the choice of the remaining coefficients $\lambda_x$ and $\gamma_y$ are arbitrary.
		Remember our goal is to find out what $(z,1)$ makes these $(u,t)$ one-dimensional. If $S_-\cap H$ was non-empty, then by setting all $\lambda_x=0$ one can make $t$ negative. If $S_+\cap H$ contained more than one point, say $x$ and $x'$, then any conical combination of $(x,1)$ and $(x',1)$ can be $(u,t)$, which then fails to be one-dimensional. It is also impossible that $S_+\cap H=\varnothing$, since otherwise $(u,t)$ must be zero and also fails to be one-dimensional. Let $x^*$ be the unique point in $S_+\cap H$. We then have that the ray is generated by $(x^*,1)$, so $z$ must be $x^*$. The uniqueness of $x^*$ in $S_+\cap H$ means $c^Tx^*+d=0$ and $c^Tx+d>0,\forall x\in S_+,x\neq x^*$. We also have $S_-\cap H=\varnothing$, which means $c^Ty+d>0,\forall y\in S_-$. This shows $x^*\in A_+^*$. This shows extreme rays in the form of $(z,1)$ must also satisfy $z\in A_+^*$. However, all the arguments can be reversed and show that any $(z,1)$ with $z\in A_+^*$ must be extreme.
		\item The argument for the ray of the form $(z,-1)$ is similar.
		\item The same type of argument shows that no ray of the form $(z,0)$ can be extreme.
	\end{enumerate}
\end{proof}
\begin{lemma}
	$R(K_+) \subseteq \{\overline{(x,1)}, \overline{(x-y,0)}: x\in A_+^*, y\in A_-^*\}$.
	Similarly, 
	$R(K_-) \subseteq \{\overline{(-y,-1)}, \overline{(x-y,0)}: x\in A_+^*, y\in A_-^*\}$.
\end{lemma}
\begin{proof}
	symmetric blah
	\begin{claim}
		$(z,1)$ is extreme in $K_+$ if and only if $(z,1)$ is extreme in $K$.
	\end{claim}
	\begin{proof}[Proof of Claim]
	$\phantom{a}$

		``$\Leftarrow$'': The halfspace that contains $K$ also contains $K_+$. The intersection with $K$ is $\overline{(z,1)}$, which is entirely in $K_+$, hence also one-dimensional.

		``$\Rightarrow$'': Suppose $(z,1)$ is the midpoint of $(z_1,t_1)\in K$ and $(z_1,t_2)\in K$. Then $(z,1)$ is also the midpoint of $((1-\ep)z+\ep z_1,1-\ep+\ep t_1)$ and $((1-\ep)z+\ep z_2,1-\ep+\ep t_2)$. With a sufficiently small $\ep$, both points are in $K_+$. Since $(z,1)$ is extreme in $K_+$, the two points must be a scaling of $(z,1)$. Hence $(z_1,t_1)$ and $(z_1,t_2)$ are also scalings of $(z,1)$. This shows $(z,1)$ is extreme in $K$.
	\end{proof}

		We are left to show if $(z,0)$ is extreme then it takes the form $(x-y,0)$ with $x\in A_+^*, y\in A_-^*$. We need a further characterization of $(z,0)\in K$.
		\begin{claim}
			$(z,0)\in K_+$ if and only if $z\in \cone (S_+-S_-)$.
		\end{claim}
		In the statement we abuse the Minkowski sum notation and denote the set $\{x-y: x\in S_+,y\in S_-\}$ by $S_+-S_-$.
		To prove the claim, take the naive representation first:
	\[\textstyle(z,0)=\sum_{x\in S_+} \lambda_x(x,1)+\sum_{y\in S_-} \gamma_y(-y,-1).
	% =\left(\sum_{i,j} \lambda_ix_i-\gamma_j y_j,\sum_i\lambda_i-\sum_j\gamma_j\right)
	\]
	So $z=\sum \lambda_x x-\sum \gamma_y y$ and $\sum \lambda_x=\sum \gamma_y$.
	% where $\lambda_i,\gamma_j\geqslant0$.
	Let $\alpha=\sum \lambda_x=\sum \gamma_y$. Note that $\alpha\neq0$ unless $z=0$. We claim that
	\[z=\sum_x \lambda_x x-\sum_y \gamma_y y=\sum_{x,y} \frac{\lambda_x\gamma_y}{\alpha}\cdot(x-y)\]
	This can be seen by comparing the coefficients of each $x$ and $y$, and the proof of the claim is complete.

	We showed that $K=\cone\{(x,1),x\in A_+^*,(-y,-1),y\in A_-^*\}$. Since (x-y,0)
	\begin{align*}
		(x-y,0) &= \sum_{u\in A_+^*} \lambda_u (u,1)+\sum_{v\in A_-^*} (\gamma_v+\gamma_v') (-v,-1)
	\end{align*}
\end{proof}

\section*{Mar 4}


\begin{definition}
The {\em separating hyperplanes} are $\SH(\Am,\Ap)$ with $h \in \SH(\Am,\Ap)$ satisfying $h(x) = "+"$ for $x \in \Ap$ and $h(x) = "-"$ for $x \in \Am$. 
\end{definition}

\begin{definition}
The {\em safe points} given disclosure $(\Am,\Ap)$ are 
$$
\Safe(\Am,\Ap) = \{x \in \reals^n : \forall h \in \SH(\Am,\Ap),\ h(x) = "-"\}.
$$
\end{definition}

\begin{definition}
The {\em must leak points} for $\Sm,\Sp$ are 
$$
\ML = \{x \in \Sm : x \not\in \Safe(\Sm \setminus \{x\},\Sp).
$$
\end{definition}

\begin{theorem}
    The must leak points $\ML$ are the vertices of the safe points $\Vert(\Safe(\Sm,\Sp))$. 
\end{theorem}

\begin{lemma}
\label{l:closure}
$\Safe(\cdot,\Ap)$ is closed under $\Conv$, $\Verts$, and itself:
$$
\Safe(A,\Ap) = \Safe(\Conv(A),\Ap) = \Safe(\Verts(A),\Ap) = \Safe(\Safe(A,\Ap),\Ap).
$$
\end{lemma}

\begin{proof}
    By the hyperplane definition of $\Safe$.
\end{proof}

\begin{lemma}
\label{l:strict}
$\Safe$ is strictly smaller when its vertices are removed:
$$
V = V' \sqcup \{x\} = \Verts(\Safe(V,\Ap)) \Rightarrow \Safe(V',\Ap) \subsetneq \Safe(V,\Ap).
$$
\end{lemma}

\begin{proof}
    By the hyperplane definition of $\Safe$.
\end{proof}

\begin{proof}[Proof of theorem:]
Fix $x \in \Sm$.

If $x \not\in \Verts(\Safe(\Sm,\Sp))$:
\begin{itemize}
    \item Then by \Cref{l:closure},  $x \in \Safe(\Verts(\Safe(\Sm,\Sp))) = \Safe(\Verts(\Safe(\Sm,\Sp) \cup \Sm \setminus \{x\},\Sp),\Sp) 
    = \Safe(\Sm \setminus \{x\},\Sp)$
    \item Then, $x \not \in \ML$.
\end{itemize}

If $x \not \in \ML$:
\begin{itemize}
    \item Then, $x \in \Safe(\Sm \setminus \{x\},\Sp)$
    \item Then, $\Safe(\Sm \setminus \{x\},\Sp) = \Safe(\Sm,\Sp)$
    \item Then, by \Cref{l:strict} and contradiction, $x \not \in \Verts(\Safe(\Sm,\Sp))$
\end{itemize}
\end{proof}


\section*{Mar 1}
Bob has only query access to the labels. If Bob had a classifier then TTP can simply ask Bob for it and obtains all relevants.

Bob probably also wants to minimize \# query calls beyond relevant cases. That is, for irrelevant emails, Alice doesn't want to reveal and Bob doesn't want to look at.

TTP trusts Bob's labels.
TTP trusts Alice's $S$.
TTP doesn't trust Alice's labels ($+$ for $A_+$, $-$ for $A_-$ and irrelevant for everything else).

\section*{Feb 28}
A new protocol
\begin{algorithm}
\caption{Protocol}\label{alg:protocol}
\begin{algorithmic}[1]
% \Require $n \geq 0$
% \Ensure $y = x^n$
\State Alice picks $A_+\subseteq X$ and $A_-\subseteq X$ and sends them to TTP and Bob
\State Bob verifies that $A_+$ and $A_-$ are consistent with $h^*$, i.e. $h^*(x_+)>0, \forall x_+\in A_+$ and $h^*(x_-)>0, \forall x_-\in A_-$, and sends the result to TTP.
% \While{$N \neq 0$}
\If{Consistent}
    \State TTP computes and sends to Bob all emails potentially relevant and hidden by Alice, namely
    \[\Leak(A_+,A_-)=\{x\in S: \exists h\in\cH, h(x)>0 \text{ and consistent with }A_+ \text{ and } S\backslash A_+\}.\]
    \State Bob checks if $h\mid_{\Leak(A_+,A_-)}<0$
    \If{$h\mid_{\Leak(A_+,A_-)}<0$}
    \State Terminate with success
    \Else
    \State Bob informs TTP that Alice hid emails.
    \State TTP sends $S$ to Bob
    \EndIf
    % \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
\Else
	\State TTP sends $S$ to Bob
\EndIf
% \EndWhile
\end{algorithmic}
\end{algorithm}

\section*{2022/02/22 (= Jan 22 lunar), Tue} % (fold)
\label{sec:2022_02_22_jan_22_lunar_tue}

% section 2022_02_22_jan_22_lunar_tue (end)

Let $S_+\subseteq X$ be the set of relevant emails and $S_-\subseteq X$ be the set of irrelevant emails. Both sets are finite and we let $S=S_+\cup S_-$. Let $\cH$ be a set of real-valued functions on $X$. We assume the data $S_+$ and $S_-$ are \emph{realizable} with respect to $\cH$, which means that there exists $h^*\in\cH$ such that for each $x_+\in S_+$, $h^*(x_+)>0$ and for each $x_-\in S_-$, $h^*(x_-)<0$.

\djs{Need a who knows what section and why we model it this way.}

\begin{algorithm}
\caption{Protocol}\label{alg:protocol}
\begin{algorithmic}[1]
% \Require $n \geq 0$
% \Ensure $y = x^n$
\State Alice picks $A_+\subseteq X$ and $A_-\subseteq X$ and sends them to TTP and Bob
\State Bob verifies that $A_+$ and $A_-$ are consistent with $h^*$, i.e. $h^*(x_+)>0, \forall x_+\in A_+$ and $h^*(x_-)>0, \forall x_-\in A_-$, and sends the result to TTP.
% \While{$N \neq 0$}
\If{Consistent}
    \State TTP computes and sends to Bob all emails potentially relevant and hidden by Alice, namely
    \[\Leak(A_+,A_-)=\{x\in S: \exists h\in\cH, h(x)>0 \text{ and consistent with }A_+ \text{ and } A_-\}.\]
    % \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
\Else
	\State Terminate
\EndIf
% \EndWhile
\end{algorithmic}
\end{algorithm}

$\Pass(A_+,A_-)$ is the set of emails ``passively leaked'' by TTP.
Alice's goal is to minimize the total number of emails that are actively and passively revealed to Bob, namely
\[|\Leak(A_+,A_-)\cup A_+ \cup A_-|\tag{*}.\]
\begin{theorem}
	The minimizer of $(*)$ is $A_+^*=S_+$ and
    \[A_-^*=\{x\in S_-: \exists h\in\cH, h\mid_{S_-\backslash\{x\}}\leqslant0,h(x)=0,h\mid_{S_+}>0\}.\]
\end{theorem}
In particular, Alice is incentivized to send all relevant emails.

\djs{Provide an upper bound of $|A_-^*|$ for special cases?}

\djs{Re-write proof}
\begin{proof}
	Observe that for any variables $A_+\subseteq S_+,A_-\subseteq S_-$
\begin{itemize}
	\item $\Leak(A_+,A_-)$ is decreasing in both variables
\end{itemize}
And because of realizability,
\begin{itemize}
	\item $\Leak(A_+,A_-)\supseteq S_+$
\end{itemize}
We have
\begin{align*}
	\Leak(A_+,A_-)\cup A_+ \cup A_-
	&=\Leak(A_+,A_-)\cup A_-\\
	&\supseteq\Leak(S_+,A_-)\cup A_-\\
	&=S_+\sqcup L(A_-)\sqcup A_-
\end{align*}
where $L(A_-)=\Leak(S_+,A_-)\backslash S_+\subseteq S_-$. Note that by definition $L(A_-)$ and $A_-$ are disjoint.

% Let $A_-'=L(A_-)\sqcup A_-$ then we have $L(A_-)\sqcup A_- = L(A_-')\sqcup A_-'$. In fact, $L(A_-')=\varnothing$.
% \begin{itemize}
% 	\item $L(L(A)\sqcup A)=\varnothing$\\
% 	In particular, let $A'=L(A)\sqcup A$ then we have $L(A)\sqcup A = L(A')\sqcup A'$. Hence we can restrict to $A$ such that $L(A)=\varnothing$.
% \end{itemize}
The optimality of $A_-^*$ is the consequence of the following two lemmas.
\begin{lemma}
	$A_-^*\subseteq L(A)\sqcup A, \forall A\subseteq S_-$.
\end{lemma}
\begin{proof}
	First we claim that $A_-^*=\{x\in S_-:L(S_-\backslash\{x\})=\{x\}\}$. It's almost a tautology. Then the lemma follows from the monotonicity of $L$.
\end{proof}
% Note that for most $x$, $L(S_-\backslash\{x\})=\varnothing$.
\begin{lemma}
	$L(A_-^*)=\varnothing$.
\end{lemma}
\begin{proof}
?
	% Let $x\in L(A_-^*)$. We know $L(A_-)$ and $A_-$ are disjoint for any $A_-\subseteq S_-$, so $x\not\in A_-^*$ and equivalently, $A_-^*\subseteq S_-\backslash\{x\}$. Since $x\not\in A_-^*$, we have $L(S_-\backslash\{x\})=\varnothing$. On the other hand we have $A_-^*\subseteq S_-\backslash\{x\}$, so by monotonicity,
	% \[L(A_-^*)\subseteq S_-\backslash\{x\}\]
\end{proof}
% \begin{proof}
% 	It sufficies to show if $x\not\in A$ then $x\in B\implies x\in L(A)$.
% 	Since $x\not\in A$, we have $A\subseteq S_-\backslash \{x\}$. By monotonicity, we have $L(A)\supseteq L(S_-\backslash \{x\})=\{x\}$, which is $x\in L(A)$.
% \end{proof}
\end{proof}

\newpage

\section*{Feb 19}

Let
\[\Leak(A_+,A_-)=\{x\in S: \exists h\in\cH \text{ consistent with }A_+\text{ and }A_- \text{ and } h(x)=+1\}\]
The goal is to minimize
\[|\Leak(A_+,A_-)\cup A_+ \cup A_-|\]
Observe that
\begin{itemize}
	\item $\Leak(A_+,A_-)\supseteq S_+$
	\item $\Leak(A_+,A_-)$ is decreasing in both variables
\end{itemize}
We have
\begin{align*}
	\Leak(A_+,A_-)\cup A_+ \cup A_-
	&=\Leak(A_+,A_-)\cup A_-\\
	&\supseteq\Leak(S_+,A_-)\cup A_-\\
	&=S_+\sqcup L(A_-)\sqcup A_-
\end{align*}
where $L(A_-)=\Leak(S_+,A_-)\backslash S_+$.
Observe that
\begin{itemize}
	\item $L(L(A)\sqcup A)=\varnothing$\\
	In particular, let $A'=L(A)\sqcup A$ then we have $L(A)\sqcup A = L(A')\sqcup A'$. Hence we can restrict to $A$ such that $L(A)=\varnothing$.
	\item 
\end{itemize}
Let $B=\{x:L(S_-\backslash\{x\})=\{x\}\}$. Note that for most $x$, $L(S_-\backslash\{x\})=\varnothing$.
We have
\begin{lemma}
	$B\subseteq L(A)\sqcup A, \forall A\subseteq S_-$.
\end{lemma}
\begin{proof}
	It sufficies to show if $x\not\in A$ then $x\in B\implies x\in L(A)$.
	Since $x\not\in A$, we have $A\subseteq S_-\backslash \{x\}$. By monotonicity, we have $L(A)\supseteq L(S_-\backslash \{x\})=\{x\}$, which is $x\in L(A)$.
\end{proof}
If $L(B)=\varnothing$ then $B$ is an (abstract) minimizer. Do we use the property of linear classifier here?

\section{Sep 10}
\newcommand{\err}{\mathrm{err}}
Separable:
\begin{itemize}
	\item Bob confirms $\err(A)=0$
	\item TTP computes $\Leak(A)=\{x:\err((x,+)\cup A)=0\}$
\end{itemize}
Nonseparable:
\begin{itemize}
	\item Bob confirms $\err_f(A)=0$
	\item TTP computes $\err_\cH(A)=k$
	$\Leak(A)=\{x:\err((x,+)\cup A)=k\}$
\end{itemize}
\section{Sep 2}

Consider the larger machine learning problem:
\begin{enumerate}
    \item Alice gives all the data $N$ to TTP.
    \item TTP picks a sample of the data $S$
    \item Insert protocol here:
    \begin{enumerate}
        \item Alice labels a subset of $S$ as $S_+$ and $S_-$.
        \item TTP gives Leak($S_+ \cup S_-$) to Bob
        \item Bob verifies accuracy of $S_+$ and $S_-$
    \end{enumerate}
    \item Bob chooses a classifier $h$ consistent with $S_+$ and $S_-$.
    \item TTP gives $N_h = \{x \in N : h(x) = +\}$ to Bob (positive points of $N$ according to $h$)
\end{enumerate}

Make sure Alice and Bob agree on the feature maps/RKHSs

\section{Aug 25} % (fold)
Let $X=\R^d$ and $\cH$ be the class of all affine functions. Suppose $S\subseteq X$ is in general position, i.e. no $d+1$ points in $S$ lie in a hyperplane. $S$ is labeled by $h^*\in\cH$ and divided into $S_+=\{x\in S: h^*(x)> 0\}$ and $S_-=\{x\in S: h^*(x)< 0\}$.
Let
\[B:=\{x\in S_-: \exists h\in\cH\text{ consistent with }S, h(x)=0\}\]
\begin{theorem}
	$B$ is a minimizer of $f$.
\end{theorem}
Observation: 1. for any $x\in B$, if $x\not\in C$ then $x\in\Leak(C)$ 2. $\Leak(B)=B$.

Next steps:
\begin{itemize}
	\item Computation: How to find $B$ quicker than running $n$ linear programmings of size $n\times d$?
	\item TTP computing T is also as expensive. Can Alice provide a short proof that $\Leak(A)=A$?
	\item Beyond realizable case?
\end{itemize}

\section{Aug 19} % (fold)
\begin{itemize}
	\item $A\nearrow, T_A\searrow$
	\item $T_A\supseteq S_+$
	\item Goal: minimize $(A\cup T) \cap S_- = (A\cap S_-)\cup (T\cap S_-)$
	\item Obviously the minimizer $A\supseteq S_+\cup S_0$. The variable becomes $B\cap S_-$ where $A = S_+\cup S_0\cup B$
	\item For $B\subseteq S_-$, let $\Leak(B) = B\cup (T\cap S_-)$ be the objective.
	\item We know $\Leak(S_-)=S_-$.
	\item In addition, $\Leak(\Leak(B))=\Leak(B)$. In fact,
	\[\Leak(\Leak(B))=\Leak(B)\cup T_{\Leak(B)} = B\cup T_B \cup T_{\Leak(B)}= B\cup T_B = \Leak(B)\]
	since $\Leak(B)\supseteq B$ and $T_B\searrow$.
	\item Goal: minimize $f(B) = |\Leak(B)|$. It suffices to minimize $f$ over the fixed points of $\Leak$, because $f(\Leak(B))=f(B)$ and $\Leak(B)$ is a fixed point of $\Leak$.
	\item $f$ is neither submodular nor supermodular.
	\item For $\mathcal{H}$ there is a mixed-integer program that minimizes $f(B)$
\end{itemize}
Protocol 1:
\begin{enumerate}
	\item Alice sends $A\subseteq X\times \R$ to TTP and Bob
	\item TTP computes\[T=\{x\in S: \exists h\in\cH \text{ consistent with }A \text{ and } h(x)=+1\}\] and sends $T$ to Bob
\end{enumerate}
Several desired outcomes:
\begin{itemize}
	\item $S_+\subseteq \Pi_X A\cup T$. Bob is happy.
	\item $(\Pi_X A\cup T)\cap S_- = \varnothing$. Alice has privacy.
	\item $S_+\nsubseteq\Pi_X A\cup T$. Alice hides.
	\item $A\nsubseteq G(f)$. Alice lies.
\end{itemize}
\begin{lemma}
The following two are equivalent:
\begin{enumerate}
	\item 
	If TTP is honest, then either Bob is happy with $T$ and Alice has privacy or Bob discovers Alice's lie using $A$.
	\item If $h\in\cH, h|_{S_+} = +1, h|_{S_0} = 0$ then $h|_{S_-}\in\{-1,0\}$.
\end{enumerate}
\end{lemma}
\begin{proof}
	If Alice doesn't lie, then $\Pi_X A\subseteq T$ and $S_+\subseteq T$. Bob is happy with $T$.
	If $A$ is very small (or large but has little information), then $T$ not only contains $S_+$ but also $S_-$ and ruins Alice's privacy. Alice would like to provide $S_+\cup S_0$.
\end{proof}
Current problem: It's unfair to Alice if even though she sends everything honestly TTP still leaks her privacy. That depends on $S$ and $\mathcal{H}$.

Question: If $\cH$ is the linear classifiers, what $S$ protects Alice's privacy?

General intuition:
$S_+$ has to be more ``informative'' about the boundary than $S_-$. Informative could mean 1. close to the boundary ($w$) 2. spans a wide are ($w^{\perp}$)

A conjecture:
\[\min_{x\in S_+} w^Tx> \max_{x\in S_0} w^Tx\implies \max_{x\in S_0} w^Tx> \max_{x\in S_-} w^Tx\]

$X=\R^d, S\sim N(0,I_{d\times d})$ $f:X\to\{\pm,0\}$ is generated by unit vector $w^*$ $f(x)= \chi( {w^*}^Tx)$
\newpage
Protocol 2:
\begin{enumerate}
	\item Alice sends the positives $S_{(0,1)}$ in $S_0$ to TTP and Bob (assuming $f\in\R^X$)
	\item Bob finds $\hat{f}\in\cH$ consistent with $S_{(0,1)}$ and sends a description of $\hat{f}$ to TTP
	\item TTP sends $S\cap \hat{f}^{-1}(+1)$ to Bob
\end{enumerate}

What if Bob only has $f:X\to\{\pm1\}$?



\section{Notes: to be removed}
State upfront in the setting: Bob is honest; he cannot lie about labels since Alice can check, and can go to court if there is a disagreement. 

Machine learning framework is an outer wrapper. 

Protocol for a given dataset $S \subseteq U$. 

\begin{enumerate}
    \item (Correct) Bob always receives $S_+$
    \item (Minimal) Alice minimizes privacy loss (reveals as few negative examples as possible to Bob).
    \item (Efficiently implementable): All algorithms (including TTP) are efficiently implementable. 
    \item (Optional: truthfulness / direct): revealing S+ minimizes S- that are disclosed (the points alice reveals are the points bob sees)
\end{enumerate}

can write a revelation principle: given correct non-truthful mechanism M with alice's minimal strategy s given data (S+,S-):
\begin{enumerate}
\item Alice reports S+
\item TTP simulates M(s(S+))
\end{enumerate}
Thm: M' is correct, truthful.




To name: points that must be disclosed even if everything else is disclosed "critical points"

Results:
\begin{enumerate}
    \item thm: any correct protocol discloses critical points.
    \item thm: critical points protocol: if alice discloses critical points, then only critical points are disclosed, any other disclosure results in at least the critical points being disclosed. ("truthfulness")
    \item corollary: critical points protocol is correct and minimal.
\end{enumerate}




==> geom.tex <==
%!TEX root = e-disc.tex


\section{Geometry of Binary Linear Classification}
\djs{replace $A_+^*$}
Given two finite sets $S_+$ and $S_-$ in $\R^n$,
let $K_{S_+,S_-}=\cone\{(x,1),x\in S_+,(-y,-1),y\in S_-\}$. Recall that $\cone(A)$ consists of non-negative linear combination of points in $A$. Hence $K_{S_+,S_-}$ is a convex cone in $\R^{n+1}$. Its dual cone
\begin{align*}
	K^*_{S_+,S_-}:=\{w\mid \inner{w}{x} \geqslant 0, \forall x\in K_{S_+,S_-}\} =\{(c,d)\in\R^{n+1}\mid c^Tx+d&\geqslant0,\forall x\in S_+\\
	c^Tx+d&\leqslant0,\forall y\in S_-\}
\end{align*}
consists of linear classifiers consistent with $S_+$ and $S_-$.

Notice that $S_+$ anb $S_-$ are linear separable if and only if $K^*_{S_+,S_-}\neq \{0\}$, which is equivalent to that $K_{S_+,S_-}=\R^{n+1}$. \djs{Not quite true in the degenerate case...}
% , i.e. $K^*_{S_+,S_-}=\cH_{S_+,S_-}$ 

% =S\cap(H^-_{A,B})^c
Let
\begin{align*}
	A_+^* &:= \{x^*\in S_+: \exists (c,d)\text{ s.t. } c^Tx^*+d=0\text{ and }c^Tx+d>0,\forall x\in S_+,x\neq x^*\text{ and }c^Ty+d<0,\forall y\in S_-\}\\
	A_-^* &:= \{y^*\in S_-: \exists (c,d)\text{ s.t. } c^Ty^*+d=0\text{ and }c^Ty+d<0,\forall y\in S_-,y\neq y^*\text{ and }c^Tx+d>0,\forall x\in S_+\}
\end{align*}

For a convex cone $C$, let $R(C)$ be the set of extreme rays of $C$. For a point $x$, let $\overline{x}=\{\lambda x: \lambda\geqslant0\}$ be the ray represented by $x$.
\begin{lemma}\label{lem:cone}
	$R(K_{S_+,S_-}) = \{\overline{(x,1)}, \overline{(-y,-1)}: x\in A_+^*, y\in A_-^*\}$.
\end{lemma}
In particular, we have
\begin{corollary}\label{cor:coneK}
For $A_+\subseteq S_+, A_-\subseteq S_-$, 
	$K^*_{S_+,S_-}=K^*_{A_+,A_-}$ if and only if $A_+\supseteq A_+^*$ and $A_+\supseteq A_-^*$.
	% In particular,
	% $K^*_{S_+,S_-}=K^*_{A^*_+,A^*_-}$
	% $\cH_{S_+,S_-}=\cH_{A^*_+,A^*_-}$
\end{corollary}

Let
\begin{align*}
	H^+_{S_+,S_-}&=\{x:c^T x+d\geqslant 0, \forall (c,d)\in K^*_{S_+,S_-}\},\\
	H^-_{S_+,S_-}&=\{x:c^T x+d\leqslant 0, \forall (c,d)\in K^*_{S_+,S_-}\}
\end{align*}
In the separable case, these are the points whose lables have no ambiguity --- all consistent classifiers are unanimous. In fact, they have a more straightforward characterization
\begin{lemma}	
\begin{align*}
	H^+_{S_+,S_-}&=\{x:(x,1)\in K_{S_+,S_-}\},\\
	H^-_{S_+,S_-}&=\{y:(-y,-1)\in K_{S_+,S_-}\}
\end{align*}
\end{lemma}

\djs{Connecting to the protocol. Need expansion
\[\Leak(A_+,A_-)=\{z\in S: (-z,-1)\not\in K_{A_+,A_-}\}\]
}
% We demonstrate a way of using minimal information from $S_+$ and $S_-$ to reconstruct $H_+$ and $H_-$. Let

% \begin{align*}
% 	A_+^* &:= \{x^*\in S_+: \exists (c,d)\text{ s.t. } c^Tx^*+d=0\text{ and }c^Tx+d>0,\forall x\in S_+,x\neq x^*\text{ and }c^Ty+d<0,\forall y\in S_-\}\\
% 	A_-^* &:= \{y^*\in S_-: \exists (c,d)\text{ s.t. } c^Ty^*+d=0\text{ and }c^Ty+d<0,\forall y\in S_-,y\neq y^*\text{ and }c^Tx+d>0,\forall x\in S_+\}
% \end{align*}
\begin{theorem}
	\begin{align*}
		H^+_{S_+,S_-} &= \conv(A_+^*)+\cone(A_+^*-A_-^*)\\
		H^-_{S_+,S_-} &= \conv(A_-^*)+\cone(A_-^*-A_+^*)
	\end{align*}
\end{theorem}
In the statement we abuse the Minkowski sum notation and denote the set $\{x-y: x\in A_+^*,y\in A^*_-\}$ by $A^*_+-A^*_-$.
\begin{proof}
	If $z\in H^+_{S_+,S_-}$, then $(z,1)\in K$.
	By \Cref{lem:cone}, there exist positive numbers $\lambda_x,\gamma_y$ for each $x\in A_+^*$ and $y\in A_-^*$ such that
	\[\textstyle(z,1)=\sum_{x\in A^*_+} \lambda_x(x,1)+\sum_{y\in A^*_-} \gamma_y(-y,-1).
	% =\left(\sum_{i,j} \lambda_ix_i-\gamma_j y_j,\sum_i\lambda_i-\sum_j\gamma_j\right)
	\]
	So $z=\sum \lambda_x \cdot x-\sum \gamma_y \cdot y$ and $\sum \lambda_x-\sum \gamma_y=1$.
	% where $\lambda_i,\gamma_j\geqslant0$.
	Let $\alpha=\sum \gamma_y\geqslant0$. We have $\sum \lambda_x=1+\alpha$. We claim that
	\[z=\underbrace{\sum_x \frac{\lambda_x}{1+\alpha}\cdot x}_{\in \conv(A_+^*)} + \underbrace{\sum_{x,y} \frac{\lambda_x\gamma_y}{1+\alpha}\cdot(x-y)}_{\in \cone(A_+^*-A_-^*)}\]
	The identity can be seen by comparing the coefficients of each $x$ and $y$. Note that the coefficients in the first summation sum to 1: $\sum_x \frac{\lambda_x}{1+\alpha} = \frac{\sum_x\lambda_x}{1+\alpha}=1$. So the first summand indeed belongs to $\conv(A_+^*)$. And the coefficients in the second summation are all non-negative.
\end{proof}
For a convex cone $C$, let $R(C)$ be the set of extreme rays of $C$. For a point $x$, let $\overline{x}=\{\lambda x: \lambda\geqslant0\}$ be the ray represented by $x$.
\begin{lemma}
	$R(K) = \{\overline{(x,1)}, \overline{(-y,-1)}: x\in A_+^*, y\in A_-^*\}$.
\end{lemma}

\begin{proof}
	First notice that any ray in $K$ can be represented by a vector of the form $(z,1),(z,-1)$ or $(z,0)$.
	\begin{enumerate}
		\item 
		Suppose $(z,1)$ is extreme, this means there exists $(c,d)$ such that
		\begin{enumerate}
			\item $c^Tz+d=0$
			\item $c^Tu+dt\geqslant 0,\forall (u,t)\in K$.
			\item $c^Tu+dt=0, (u,t)\in K\implies t\geqslant0, u=tz$.
		\end{enumerate}
		The first two conditions mean $(z,1)$ supports a half-space that contains $K$. The third condition means $K$ intersects the hyperplane exactly at the ray.

		(b) is equivalent to that $c^Tx+d\geqslant 0,\forall x\in S_+,c^Ty+d\leqslant 0,\forall y\in S_-$.

		Consider $(u,t)$ in the intersection, i.e. $c^Tu+dt=0, (u,t)\in K$. We know
		$$\textstyle(u,t)=\sum_{x\in S_+} \lambda_x (x,1)+\sum_{y\in S_-} \gamma_y (-y,-1)\text{ where }\lambda_x\geqslant0,\gamma_y\geqslant0.$$
		% Hence $u=\sum_{x\in S_+} \lambda_x x-\sum_{y\in S_-} \gamma_y y$ and $t=\sum_{x\in S_+} \lambda_x-\sum_{y\in S_-} \gamma_y$ 
		Hence $u=\sum \lambda_x x-\sum \gamma_y y$ and $t=\sum \lambda_x-\sum \gamma_y$ where the obvious summation subscripts are dropped for brevity. $c^Tu+dt=0$ can be expanded as
		\begin{align*}\textstyle
			c^T\sum \lambda_x x-\sum \gamma_y y + d\cdot(\sum \lambda_x-\sum \gamma_y)=0
		\end{align*}
		\begin{align*}\textstyle
			\sum \lambda_x (c^Tx+d)=\sum \gamma_y (c^Ty + d) \tag{$*$}
		\end{align*}
		By (2), LHS of $(*)$ $\geqslant0$ and RHS of $(*)$ $\leqslant0$, which implies both are 0 and the coefficients can be positive only when the corresponding linear form evaluates to 0. More precisely, let $H=\{x:c^Tx+d=0\}$ be the hyperplane. We have
		\begin{align*}
			u&=\sum_{x\in S_+\cap H} \lambda_x x-\sum_{y\in S_-\cap H} \gamma_y y\\
			t&=\sum_{x\in S_+\cap H} \lambda_x-\sum_{y\in S_-\cap H} \gamma_y
		\end{align*}
		Moreover, the choice of the remaining coefficients $\lambda_x$ and $\gamma_y$ are arbitrary.
		Remember our goal is to find out what $(z,1)$ makes these $(u,t)$ one-dimensional. If $S_-\cap H$ was non-empty, then by setting all $\lambda_x=0$ one can make $t$ negative. If $S_+\cap H$ contained more than one point, say $x$ and $x'$, then any conical combination of $(x,1)$ and $(x',1)$ can be $(u,t)$, which then fails to be one-dimensional. It is also impossible that $S_+\cap H=\varnothing$, since otherwise $(u,t)$ must be zero and also fails to be one-dimensional. Let $x^*$ be the unique point in $S_+\cap H$. We then have that the ray is generated by $(x^*,1)$, so $z$ must be $x^*$. The uniqueness of $x^*$ in $S_+\cap H$ means $c^Tx^*+d=0$ and $c^Tx+d>0,\forall x\in S_+,x\neq x^*$. We also have $S_-\cap H=\varnothing$, which means $c^Ty+d<0,\forall y\in S_-$. This shows $x^*\in A_+^*$. This shows extreme rays in the form of $(z,1)$ must also satisfy $z\in A_+^*$. However, all the arguments can be reversed and show that any $(z,1)$ with $z\in A_+^*$ must be extreme.
		\item The argument for the ray of the form $(z,-1)$ is similar.
		\item The same type of argument shows that no ray of the form $(z,0)$ can be extreme.
	\end{enumerate}
\end{proof}


==> minimal-new.tex <==
\subsection{Minimal Protocol} \label{sec:minimal}

\newcommand{\AL}{\text{AL}}

We now argue the minimality of the critical points protocol. In what follows for a given protocol $\pi$, there are potentially several rounds of interaction between Alice, Bob and \TTP (the trusted third party). Alice takes some actions $\AL$ and Bob is asked by the \TTP to provide some labels for some points  %$\sigma$ for some points 
(which are in turn a function of $S, \AL$). 
We will denote by $\obs_\pi = \obs_\pi(S, \AL) \subset S$ to be the set of points that are revealed to Bob eventually, and corresponds to the output of the protocol. We prove that any protocol $\pi$ that is {\em correct} must have revealed the critical points $C^*(S_+)$ to Bob i.e., $C^*(S_+) \subseteq \obs_\pi$. %, where $\obs_\pi$ denotes all the samples seen by (or revealed to) Bob. 
Recall that correctness of the protocol is the guarantee that for any data set $S = (S_+, S_-)$ and any action $\AL$ of Alice, Bob sees $S_+$ (Bob may potentially receive other data points as well). We make one other natural assumption about the protocol $\pi$: the only labels that the protocol depends on are the labels provided by Bob (since there is no way for the trusted third-party \TTP to verify the correctness of the labels of the other points). In particular, while the protocol depends on $S$, it cannot depend on the partition $S_+, S_-$ (unless Bob labels all of $S$). Note that the critical points protocol satisfies all these properties. 

%Specifically, though some margin based classifiers, such as support vector machines, are supported on a subset of $\Aps \cup \Ams$; the protocol must have Bob label at least the full set $\Aps \cup \Ams$ otherwise it is not always correct.  Thus, our protocol where Bob
%labels only the full set $\Aps \cup \Ams$ is optimal.

\begin{proposition}\label{prop:minimal}
In the above notation, consider any protocol $\pi$ where Alice, \TTP, and Bob interact, satisfying
  \begin{enumerate}
     \item[(i)] {\em Correct} i.e., for any realizable labeling of $S$ into $S_+, S_-$ and any action $\AL$ of Alice, we have that $S_+$ is revealed to Bob i.e., $S_+ \subseteq \obs_\pi(S_+, S_-, \AL)$.  
     \item[(ii)] $\obs_\pi(S_+, S_-, \AL) = \obs_\pi (S_+ \cup S_-, \AL)$ i.e., the only labels that the output depends on are provided by Bob. 
  \end{enumerate}
  Then it holds that for every realizable labeling $S_+, S_-$, every action $\AL$ of Alice, $\obs_\pi(S_+, S_-, \AL) \supseteq C^*(S_+)$, where $C^*(S_+)$ is the set of vertices of $S_-$ w.r.t the classifiers $\cH_{S_+, S_-}$.  
  
%  Bob eventually labels the set $A$ as $\Ap \cup \Am$; and Bob picks a hypothesis $h \in  \SH(\Am,\Ap)$.  Then $\Am \supseteq \Ams$ and $\Ap \supseteq \Aps$.
\end{proposition}

\begin{proof}
  Suppose not, i.e., in this correct protocol $\pi$ there exists $S = \Sp \cup \Sm$, where Alice, \TTP, and Bob interact, 
  %and Bob eventually labels $A$ as $\Ap \cup \Am$; Bob picks a hypothesis $h \in \SH(\Am,\Ap)$; but $\Am \not\supseteq \Ams$ (the case of $\Ap \not\supseteq \Aps$ is symmetric).  
  and there exists $x^* \in \Ams \setminus \obs_\pi(S_+, S_-, A)$. Let $S'_+ = S_+ \cup \{ x^*\}$ and $S'_- = \Sm \setminus \{x^*\}$. Since $x^* \in C^*(S_+)$ is a vertex, $S'_+, S'_-$ is also realizable. 
  
  Consider the output of the protocol $\obs_\pi(S'_+, S'_-, \AL)$. 
  The \TTP has to guarantee correctness 
  regardless of Alice's action $\AL$. Hence $S'_+ \subseteq \obs_\pi(S'_+, S'_-, \AL)$. In particular $x^*$ is revealed to Bob.   But from condition (ii) of the protocol, $\obs_\pi(S'_+, S'_-, \AL) = \obs_\pi(S_+, S_-, \AL)$ since $S_+ \cup S_- = S'_+ \cup S'_-$. Hence $x^* \in \obs_\pi(S_+, S_-, \AL)$ which gives a contradiction, as required. 
  \end{proof}



==> minimal.tex <==
\subsection{Minimal Protocol}

In this section we prove that any protocol which guarantees that Bob
selects a valid classifier must have Bob label $\Aps$ and $\Ams$.
Specifically, though some margin based classifiers, such as support
vector machines, are supported on a subset of $\Aps \cup \Ams$; the
protocol must have Bob label at least the full set $\Aps \cup \Ams$
otherwise it is not always correct.  Thus, our protocol where Bob
labels only the full set $\Aps \cup \Ams$ is optimal.

\begin{proposition}
  Consider any protocol that is correct for any realizable labeling of
  $S$ where Alice, {\TTP}, and Bob interact; Bob eventually labels the
  set $A$ as $\Ap \cup \Am$; and Bob picks a hypothesis $h \in
  \SH(\Am,\Ap)$.  Then $\Am \supseteq \Ams$ and $\Ap \supseteq \Aps$.
\end{proposition}

\begin{proof}
  Suppose not, i.e., in this correct protocol there exists $S = \Sm
  \cup \Sp$, where Alice, {\TTP}, and Bob interact; and Bob eventually
  labels $A$ as $\Ap \cup \Am$; Bob picks a hypothesis $h \in
  \SH(\Am,\Ap)$; but $\Am \not\supseteq \Ams$ (the case of $\Ap
  \not\supseteq \Aps$ is symmetric).  Let $x \in \Ams \setminus \Am$.
  Note that {\TTP} is responsible for guaranteeing correctness
  regardless of what Alice does.  Since the {\TTP} does not query Bob on
  $x$, all parties would behave identically when Alice behaves as she
  has done to get this outcome independently of whether we are in the
  case where $x$ is ``$+$'' and or that where $x$ is ``$-$''.

  In our protocol Bob chooses an $h \in \SH(\Ap,\Am)$.  Consider the
  feasible hyperplanes in the case where $x$ is ``$+$'' and ``$-$''.
  These are $\SH(\Am \cup \{x\},\Ap)$ and $\SH(\Am,\Ap \cup \{x\})$.
  Since $x \in \Ams$, both of these sets of hyperplanes are non-empty
  (see \Cref{l:non-empty-SH}, below); thus, either labeling of $x$ is realizable.
  \Cref{l:empty-intersection}, below, shows that the intersection of
  these feasible hyperplanes is empty.  Thus, one of these sets does
  not contain Bob's selected hyperplane $h$.  Consider the labeling of
  $x$ that gives this set of hyperplanes.  On this labeling of $S$,
  Alice has a strategy where Bob chooses aninfeasible hyperplane.
  This contradicts the correctness of the protocol, and the proof by
  contradiction is complete.
\end{proof}

\begin{lemma}
\label{l:empty-intersection}
  For $\Am, \Ap, \{z\} \subset \reals^n$, then $\SH(\Am \cup \{z\},\Ap) \cap \SH(\Am,\Ap \cup \{z\}) = \emptyset$.
\end{lemma} 

\begin{proof}
  Given a direction $d$ and implicit sets $\Am$ and $\Ap$, let $C(d)$
  be the constants such that $(d,c)$ defines a separating hyperplace as $\{x \in \reals^n : d \cdot x = c\}$, i.e.,
  \begin{align*}
  C(d) &= \{c \in \reals : \xm \in \Am,\ \xp \in \Ap,\ d \cdot \xm \leq c < d \cdot \xp\}.\\
  \intertext{One way to define the separating hyperplaces $\SH(\Am,\Ap)$ is as}
  \SH(\Am,\Ap) &= \{x \in \reals^n : d \in \reals^n, \ c \in C(d), \ d \cdot x = c \}.\\
   \intertext{Thus, it is sufficient to show the lemma that $C_-(d) \cup C_+(d) = \emptyset$ where $C_-$ and $C_+$ are defined like $C$ but with respect to adding $z$ to $\Am$ and $\Ap$, respectively.  Note that:}
   C_-(d) &= C(d) \cap [d\cdot z, \infty)\\
     C_+(d) &= C(d) \cap (-\infty,d\cdot z)
  \end{align*}
  Thus, we see that $C_-(d) \cap C_+(d) = \emptyset$.
\end{proof}


\begin{lemma}
  \label{l:non-empty-SH}
  Consider labeled data $S = \Sm \sqcup \Sp$, negative examples $\Am \subseteq \Sm$, positive examples $\Ap \subseteq
  \Sp$ and required disclusure $x \in \Ams$.  Then, the sets of separating hyperplaces for either labeling of $x$, i.e., $\SH(\Am \cup \{x\},\Ap)$ and
  $\SH(\Am,\Ap \cup \{ x\})$, are non-empty.
\end{lemma}

\begin{proof}
  $\Ams$ is defined as the subset of $\Sm$ that are ambiguous when all
  other points are labeled, i.e., for $x \in \Ams$, some hyperplanes
  in $\SH(\Sm \setminus \{x\},\Sp)$ label $x$ as ``$+$'' and some as
  ``$-$''.  Thus, for either labeling, there are consistent
  hyperplanes.
\end{proof}


==> prelims.tex <==
- Single Agent Version (SPeD). \\
- Linear classification (SVM). 

Jinshuo may add: formal definitions if necessary. 


\begin{itemize}
	% \item The labels from Alice can be assume to be true.
	% \item Given that, we may as well assume that Bob is not involved in the protocol
	\item Alice has full information. She doesn't learn anything from the interaction with TTP. So she may as well just send a single message. The only thing that TTP doesn't know is the labels. So the message must be a partial labeling. Therefore, the protocol can be simplified to be at most three-round:
	\begin{enumerate}
		\item Alice sends a partial labeling to TTP
		\item TTP sends the labeled data to Bob. If Bob agree with the labels, proceed to the next step; otherwise Alice and Bob go to court and settle the labeling issue there. Then TTP use the correct labels and proceed to the next step
		\item TTP generates a set and sends to Bob. This is what Bob uses for ML.
	\end{enumerate}
	In fact, the protocol can be equivalently made two-round if the set TTP generates contains everything Alice has labeled. 
	\begin{enumerate}
		\item Alice sends a partial labeling to TTP
		\item TTP generates a (partially? labeled?) set that contains everything Alice has labeled and sends to Bob.
		If Bob agrees with the labels, then this is what Bob uses for ML; otherwise Alice and Bob go to court and settle the labeling issue there. Then TTP uses the correct labels and repeats step 2
	\end{enumerate}

	\item The only thing that TTP doesn't know is the labels. Over potentially many steps, TTP collects a partial labeling from Alice, and eventually pass a (labeled?) subset to Bob. In other words, we can assumed Alice only send a single message, which is a partial labeling, to TTP. Then TTP generates a (labeled? partially?) subset and send to Bob. If Bob agree with the labels, then that's what he uses for ML; if he doesn't, then Alice and Bob go to court and settle the labeling issue there.
\end{itemize}


A protocol on an (unlabeled) dataset $S$ is $\cM:\{+1,0,-1\}^S\to 2^S$.

A protocol $\cM$ is correct with respect to $\cH$ if for any $f:S\to\{+1,0,-1\}$, $\cM$ satisfies
\[\cM(f)\supseteq\{x:\exists h\in \cH, h\cdot f\geqslant 0, h(x)=+1\}\]

For a fixed $h\in \cH$, $S$ is labeled as $S_+$ and $S_-$ and we have the associated $A_-^*$. We have
\begin{lemma}
	For any $f:S\to\{+1,0,-1\}$ such that $h\cdot f\geqslant 0$, we have
	\[\{x:\exists h\in \cH, h\cdot f\geqslant 0, h(x)=+1\}=S_+\cup A_-^*\]
\end{lemma}

A protocol is direct if it bans partial labelings.

Privacy loss of Alice is determined by the true labeling $h$ and the action of Alice:
$\loss_\cM(h,f)=|\cM(h)\cap S_-|$.

Knowing $\cM$ and $h$, Alice takes an action $f^*$ such that
\[
f^*=f^*(\cM,h)=\argmin_{f}\loss_\cM(h,f)
\]

A protocol $\cM^*$ is optimal with respect to $\cH$ if $\cM^*$ is correct w.r.t. $\cH$ and the privacy loss of Alice is always the least possible for any ground truth label $h$, i.e.
\[
	\min_f \loss_{\cM^*}(h,f)= \min_{\cM \text{ correct}} \min_f \loss_{\cM}(h,f), \forall h\in \cH.
\]
\begin{lemma}[Revelation Principle]
	For any protocol $\cM$, there is a direct protocol $\widetilde{\cM}$ that
	\begin{enumerate}
		\item $\min_f \loss_{\widetilde{\cM}}(h,f)=\min_f \loss_{\cM}(h,f)$
		\item $\widetilde{\cM}$ is correct if $\cM$ is correct.
	\end{enumerate}
\end{lemma}
